CoFiNet: Reliable Coarse-to-fine Correspondences for Robust Point Cloud Registration

We study the problem of extracting correspondences between a pair of point clouds for registration. For correspondence retrieval, existing works benefit from matching sparse keypoints detected from dense points but usually struggle to guarantee their repeatability. To address this issue, we present CoFiNet - Coarse-to-Fine Network which extracts hierarchical correspondences from coarse to fine without keypoint detection. On a coarse scale and guided by a weighting scheme, our model firstly learns to match down-sampled nodes whose vicinity points share more overlap, which significantly shrinks the search space of a consecutive stage. On a finer scale, node proposals are consecutively expanded to patches that consist of groups of points together with associated descriptors. Point correspondences are then refined from the overlap areas of corresponding patches, by a density-adaptive matching module capable to deal with varying point density. Extensive evaluation of CoFiNet on both indoor and outdoor standard benchmarks shows our superiority over existing methods. Especially on 3DLoMatch where point clouds share less overlap, CoFiNet significantly outperforms state-of-the-art approaches by at least 5% on Registration Recall, with at most two-third of their parameters.

==> broader_impact.tex <==
\section*{Broader Impact}

Our paper presents a novel deep neural network that leverages the coarse-to-fine mechanism to extract correspondences from point clouds, which can be utilized in point cloud registration. It makes a first attempt towards the detection-free matching of point clouds. Our work can contribute to a wide range of applications, such as scene reconstruction, autonomous driving, simultaneous localization and mapping (SLAM), or any others where point cloud registration plays a role. For instance, the reconstruction of indoor scenes from unlabeled RGB-D images could benefit from our method, as it can extract reliable correspondences that can be leveraged to recover the rigid transformation more precisely. Also, in autonomous driving scenarios, our methods can help agent better sense its surroundings. As our method aims at tackling a fundamental problem in computer vision, it has no direct negative outcome. Potential negative outcome might occur in the aforementioned applications where our method involves in.
